NuSTAR and multifrequency study of the two high-redshift blazars S5 0836+710 and PKS 2149-306

The most powerful blazars are the flat spectrum radio quasars whose emission is dominated by a Compton component peaking between a few hundred keV and a few hundred MeV. We selected two bright blazars, PKS 2149-306 at redshift z=2.345 and S5 0836+710 at z=2.172, in order to observe them in the hard X-ray band with the NuSTAR satellite. In this band the Compton component is rapidly rising almost up to the peak of the emission. Simultaneous soft-X-rays and UV-optical observations were performed with the Swift satellite, while near-infrared (NIR) data were obtained with the REM telescope. To study their variability, we repeated these observations for both sources on a timescale of a few months. While no fast variability was detected during a single observation, both sources were found to be variable in the X-ray band, up to 50%, between the two observations, with larger variability at higher energies. No variability was detected in the optical/NIR band. These data together with Fermi-LAT, WISE and other literature data are then used to study the overall spectral energy distributions (SEDs) of these blazars. Although the jet non-thermal emission dominates the SED, it leaves the UV band unhidden, allowing us to detect the thermal emission of the disc and to estimate the mass of the black hole. The non-thermal emission is well reproduced by a one-zone leptonic model. The non-thermal radiative processes are synchrotron, self-Compton and external Compton using seed photons from both the broad-line region (BLR) and the torus. We find that our data are better reproduced if we assume that the location of the dissipation region of the jet, R_diss, is in-between the torus, (at R_torus), and the BLR (R_torus>R_diss>R_BLR). The observed variability is explained by changing a minimum number of model parameters by a very small amount.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

